The Paradox of Motion: Evidence for Spurious Correlations in Skeleton-based Gait Recognition Models

Gait, an unobtrusive biometric, is valued for its capability to identify individuals at a distance, across external outfits and environmental conditions. This study challenges the prevailing assumption that vision-based gait recognition, in particular skeleton-based gait recognition, relies primarily on motion patterns, revealing a significant role of the implicit anthropometric information encoded in the walking sequence. We show through a comparative analysis that removing height information leads to notable performance degradation across three models and two benchmarks (CASIA-B and GREW). Furthermore, we propose a spatial transformer model processing individual poses, disregarding any temporal information, which achieves unreasonably good accuracy, emphasizing the bias towards appearance information and indicating spurious correlations in existing benchmarks. These findings underscore the need for a nuanced understanding of the interplay between motion and appearance in vision-based gait recognition, prompting a reevaluation of the methodological assumptions in this field. Our experiments indicate that "in-the-wild" datasets are less prone to spurious correlations, prompting the need for more diverse and large scale datasets for advancing the field.

==> tables/old-casia-no-gait.tex <==
\begin{table*}[hbt!]
    \caption{Results of the single skeleton model for all types of normalization techniques on the CASIA-B test set. For each setting, we show the average performance of 3 runs with different seeds. The top model manages to obtain a recognition accuracy of 57.49\% using only one pose, demonstrating that a single skeleton encodes discriminative appearance information.}
    \label{tab:no_gait_casia_old}
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ l | c | c | c | c | c | c | c | c }
        & \multicolumn{4}{c|}{\textbf{Single Skeleton}} & \multicolumn{4}{c}{\textbf{Average Prediction}} \\
         \textbf{Normalization} & \textbf{NM} &  \textbf{BG} & \textbf{CL} & \textbf{Mean} & \textbf{NM} & \textbf{BG} & \textbf{CL} & \textbf{Mean} \\
        \midrule
        \textit{Frame-scale} & \textbf{36.45} \scriptsize{$\pm$ 2.67} & \textbf{30.99} \scriptsize{$\pm$ 1.6} & \textbf{23.28} \scriptsize{$\pm$ 0.41} & \textbf{30.24} \scriptsize{$\pm$ 1.56} & 70.71 \scriptsize{$\pm$ 1.13} & 56.68 \scriptsize{$\pm$ 1.19} & 41.44 \scriptsize{$\pm$ 0.77} & 56.28 \scriptsize{$\pm$ 0.87} \\
        \textit{BBox scale} & 27.43 \scriptsize{$\pm$ 0.6} & 21.7 \scriptsize{$\pm$ 0.85} & 14.96 \scriptsize{$\pm$ 0.91} & 21.37 \scriptsize{$\pm$ 0.57} & 64.81 \scriptsize{$\pm$ 0.86} & 48.24 \scriptsize{$\pm$ 1.65} & 32.95 \scriptsize{$\pm$ 1.63} & 48.66 \scriptsize{$\pm$ 0.59} \\
        \textit{BBox-translate} & 18.35 \scriptsize{$\pm$ 1.08} & 12.55 \scriptsize{$\pm$ 0.71} & 8.72 \scriptsize{$\pm$ 0.69} & 13.21 \scriptsize{$\pm$ 0.41} & 59.53 \scriptsize{$\pm$ 1.15} & 41.19 \scriptsize{$\pm$ 0.68} & 25.05 \scriptsize{$\pm$ 0.14} & 41.93 \scriptsize{$\pm$ 0.54} \\
        \textit{BBox-translate + BBox-scale} & 19.21 \scriptsize{$\pm$ 0.53} & 13.71 \scriptsize{$\pm$ 0.4} & 8.07 \scriptsize{$\pm$ 0.14} & 13.66 \scriptsize{$\pm$ 0.17} & 60.04 \scriptsize{$\pm$ 0.54} & 39.87 \scriptsize{$\pm$ 0.76} & 21.06 \scriptsize{$\pm$ 0.97} & 40.33 \scriptsize{$\pm$ 0.29} \\
        \textit{BBox-translate + Frame-scale} & 19.93 \scriptsize{$\pm$ 0.28} & 14.68 \scriptsize{$\pm$ 0.67} & 8.95 \scriptsize{$\pm$ 0.32} & 14.5 \scriptsize{$\pm$ 0.36} & 60.07 \scriptsize{$\pm$ 0.84} & 40.76 \scriptsize{$\pm$ 0.84} & 23.4 \scriptsize{$\pm$ 0.47} & 41.41 \scriptsize{$\pm$ 0.12} \\
        \textit{BatchNorm} & 36.34 \scriptsize{$\pm$ 0.65} & 30.12 \scriptsize{$\pm$ 0.6} & 21.73 \scriptsize{$\pm$ 0.85} & 29.4 \scriptsize{$\pm$ 0.2} & \textbf{73.0} \scriptsize{$\pm$ 0.58} & \textbf{57.95} \scriptsize{$\pm$ 0.18} & \textbf{41.53} \scriptsize{$\pm$ 0.22} & \textbf{57.49} \scriptsize{$\pm$ 0.33} \\
        \textit{Avg BBox} & 35.77 \scriptsize{$\pm$ 2.05} & 29.2 \scriptsize{$\pm$ 1.92} & 22.41 \scriptsize{$\pm$ 1.06} & 29.15 \scriptsize{$\pm$ 1.67} & 72.47 \scriptsize{$\pm$ 1.66} & 57.61 \scriptsize{$\pm$ 1.4} & 39.08 \scriptsize{$\pm$ 1.2} & 56.48 \scriptsize{$\pm$ 1.24} \\
        \textit{Avg Coordinates} & 35.77 \scriptsize{$\pm$ 2.05} & 29.2 \scriptsize{$\pm$ 1.92} & 22.48 \scriptsize{$\pm$ 1.16} & 29.15 \scriptsize{$\pm$ 1.67} & 72.47 \scriptsize{$\pm$ 1.66} & 57.61 \scriptsize{$\pm$ 1.4} & 39.08 \scriptsize{$\pm$ 1.2} & 56.48 \scriptsize{$\pm$ 1.24} \\
        \end{tabular}
    }
    \end{center}
\end{table*}
